A Machine Learning Approach to Enhancing eROSITA Observations

The eROSITA X-ray telescope, launched in 2019, is predicted to observe roughly 100,000 galaxy clusters. Follow-up observations of these clusters from Chandra, for example, will be needed to resolve outstanding questions about galaxy cluster physics. Deep Chandra cluster observations are expensive and follow-up of every eROSITA cluster is infeasible, therefore, objects chosen for follow-up must be chosen with care. To address this, we have developed an algorithm for predicting longer duration, background-free observations based on mock eROSITA observations. We make use of the hydrodynamic cosmological simulation Magneticum, have simulated eROSITA instrument conditions using SIXTE, and have applied a novel convolutional neural network to output a deep Chandra-like "super observation" of each cluster in our simulation sample. Any follow-up merit assessment tool should be designed with a specific use case in mind; our model produces observations that accurately and precisely reproduce the cluster morphology, which is a critical ingredient for determining cluster dynamical state and core type. Our model will advance our understanding of galaxy clusters by improving follow-up selection and demonstrates that image-to-image deep learning algorithms are a viable method for simulating realistic follow-up observations.

==> JournalAbbrevs.tex <==
\newcommand\aj{{AJ}}% 
          % Astronomical Journal 
\newcommand\araa{{ARA\&A}}% 
          % Annual Review of Astron and Astrophys 
%\newcommand\apj{{ApJ}}% 
          % Astrophysical Journal 
\newcommand\apjl{{ApJ}}% 
          % Astrophysical Journal, Letters 
\newcommand\apjs{{ApJS}}% 
          % Astrophysical Journal, Supplement 
%\newcommand\ao{{Appl.~Opt.}}% 
          % Applied Optics 
\newcommand\apss{{Ap\&SS}}% 
          % Astrophysics and Space Science 
\newcommand\aap{{A\&A}}% 
          % Astronomy and Astrophysics 
\newcommand\aapr{{A\&A~Rev.}}% 
          % Astronomy and Astrophysics Reviews 
\newcommand\aaps{{A\&AS}}% 
          % Astronomy and Astrophysics, Supplement 
\newcommand\azh{{AZh}}% 
          % Astronomicheskii Zhurnal 
\newcommand\baas{{BAAS}}% 
          % Bulletin of the AAS 
\newcommand{\jcap}{J. Cosm. Astropart. Phys.}
	% Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{{JRASC}}% 
          % Journal of the RAS of Canada 
\newcommand\memras{{MmRAS}}% 
          % Memoirs of the RAS 
\newcommand\mnras{{MNRAS}}% 
          % Monthly Notices of the RAS 
%\newcommand\pra{{Phys.~Rev.~A}}% 
          % Physical Review A: General Physics 
%\newcommand\prb{{Phys.~Rev.~B}}% 
          % Physical Review B: Solid State 
%\newcommand\prc{{Phys.~Rev.~C}}% 
          % Physical Review C 
%\newcommand\prd{{Phys.~Rev.~D}}% 
          % Physical Review D 
%\newcommand\pre{{Phys.~Rev.~E}}% 
          % Physical Review E 
%\newcommand\prl{{Phys.~Rev.~Lett.}}% 
          % Physical Review Letters 
\newcommand\pasp{{PASP}}% 
          % Publications of the ASP 
\newcommand\pasj{{PASJ}}% 
          % Publications of the ASJ 
\newcommand\qjras{{QJRAS}}% 
          % Quarterly Journal of the RAS 
\newcommand\skytel{{S\&T}}% 
          % Sky and Telescope 
\newcommand\solphys{{Sol.~Phys.}}% 
          % Solar Physics 
\newcommand\sovast{{Soviet~Ast.}}% 
          % Soviet Astronomy 
\newcommand\ssr{{Space~Sci.~Rev.}}% 
          % Space Science Reviews 
\newcommand\zap{{ZAp}}% 
          % Zeitschrift fuer Astrophysik 
%\newcommand\nat{{Nature}}% 
          % Nature 
\newcommand\iaucirc{{IAU~Circ.}}% 
          % IAU Cirulars 
\newcommand\aplett{{Astrophys.~Lett.}}% 
          % Astrophysics Letters 
\newcommand\apspr{{Astrophys.~Space~Phys.~Res.}}% 
          % Astrophysics Space Physics Research 
\newcommand\bain{{Bull.~Astron.~Inst.~Netherlands}}% 
          % Bulletin Astronomical Institute of the Netherlands 
\newcommand\fcp{{Fund.~Cosmic~Phys.}}% 
          % Fundamental Cosmic Physics 
\newcommand\gca{{Geochim.~Cosmochim.~Acta}}% 
          % Geochimica Cosmochimica Acta 
\newcommand\grl{{Geophys.~Res.~Lett.}}% 
          % Geophysics Research Letters 
%\newcommand\jcp{{J.~Chem.~Phys.}}% 
          % Journal of Chemical Physics 
\newcommand\jgr{{J.~Geophys.~Res.}}% 
          % Journal of Geophysics Research 
\newcommand\jqsrt{{J.~Quant.~Spec.~Radiat.~Transf.}}% 
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand\memsai{{Mem.~Soc.~Astron.~Italiana}}% 
          % Mem. Societa Astronomica Italiana 
\newcommand\nphysa{{Nucl.~Phys.~A}}% 
          % Nuclear Physics A 
\newcommand\physrep{{Phys.~Rep.}}% 
          % Physics Reports 
\newcommand\physscr{{Phys.~Scr}}% 
          % Physica Scripta 
\newcommand\planss{{Planet.~Space~Sci.}}% 
          % Planetary Space Science 
\newcommand\procspie{{Proc.~SPIE}}% 
          % Proceedings of the SPIE 
\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 
